Survey on the Canonical Metrics on the Teichm\"{u}ller Spaces and the Moduli Spaces of Riemann Surfaces

This thesis results from an intensive study on the canonical metrics on the Teichm\"{u}ller spaces and the moduli spaces of Riemann surfaces. There are several renowned classical metrics on $T_g$ and $\mathcal{M}_g$, including the Weil-Petersson metric, the Teichm\"{u}ller metric, the Kobayashi metric, the Bergman metric, the Carath\'{e}odory metric and the K\"{a}hler-Einstein metric. The Teichm\"{u}ller metric, the Kobayashi metric and the Carath\'{e}odory metric are only (complete) Finsler metrics, but they are effective tools in the study of hyperbolic property of $\mathcal{M}_g$. The Weil-Petersson metric is an incomplete K\"{a}hler metric, while the Bergman metric and the K\"{a}hler-Einstein metric are complete K\"{a}hler metrics. However, McMullen introduced a new complete K\"{a}hler metric, called the McMullen metric, by perturbing the Weil-Petersson metric. This metric is indeed equivalent to the Teichm\"{u}ller metric. Recently, Liu-Sun-Yau proved that the equivalence of the K\"{a}hler-Einstein metric to the Teichm\"{u}ller metric, and hence gave a positive answer to a conjecture proposed by Yau. Their approach in the proof is to introduce two new complete K\"{a}hler metrics, namely, the Ricci metric and the perturbed Ricci metric, and then establish the equivalence of the Ricci metric to the K\"{a}hler-Einstein metric and the equivalence of the Ricci metric to the McMullen metric. The main purpose of this thesis is to survey the properties of these various metrics and the geometry of $T_g$ and $\mathcal{M}_g$ induced by these metrics.

==> bib.tex <==
\begin{thebibliography}{99}
\addcontentsline{toc}{chapter}{Bibliography}

\bibitem{bib1}
K. Liu, X. Sun and S.-T. Yau,
{\it Canonical metrics on the moduli spaces of Riemann surfaces I},
J. Diff. Geom., {\bf 68}(3): 571-637 (2004).

\bibitem{bib2}
K. Liu, X. Sun and S.-T. Yau,
{\it Canonical metrics on the moduli spaces of Riemann surfaces II},
J. Diff. Geom., {\bf69}(1): 163-216 (2005).

\bibitem{bib3}
C. T. McMullen,
{\it The moduli space of Riemann surfaces is K\"{a}hler hyperbolic},
Ann. of Math. (2), {\bf 151}(1): 327-357 (2000).

\bibitem{bib4}
L. V. Ahlfors,
{\it Conformal Invariants: Topics in Geometric Function Theory},
McGraw-Hill, New York, 1973.

\bibitem{bib5}
L. V. Ahlfors and L. Sario,
{\it Riemann Surfaces},
Princeton Univ. Press, Princeton, New Jersey, 1960.

\bibitem{bib6}
H. Farkas and I. Kra,
{\it Riemann Surfaces},
Springer-Verlag, Berlin and New York, 1980.

\bibitem{bib7}
G. Springer,
{\it Introductin to Riemann Surfaces},
Addison-Wesley, Reading, Massachusetts, 1957.

\bibitem{bib8}
L. V. Ahlfors,
{\it Curvature Properties of Teichm\"{u}ller's Space},
J. d'Analyse Math., {\bf 9}: 161-176 (1961).

\bibitem{bib9}
H. Masur,
{\it Extension of the Weil-Petersson Metric to the Boundary of Teichm\"{u}ller Space},
Duke Math. J., {\bf 43}(3): 623-635 (1976).

\bibitem{bib10}
S. Trapani,
{\it On the Determinant of the Bundle of Meromorphic Quadratic Differentials on the Deligne-Mumford Compactification of the Moduli Space of Riemann Surfaces},
Math. Ann., {\bf 293}(4): 681-705 (1992).

\bibitem{bib11}
S. A. Wolpert,
{\it The Hyperbolic Metric and the Geometry of the Universal Curve},
J. Diff. Geom., {\bf 31}(2): 417-472 (1990).

\bibitem{bib12}
S. A. Wolpert,
{\it Geodesic length functions and the Nielsen problem},
J. Diff. Geom., {\bf 25}: 275-296 (1987).

\bibitem{bib13}
G. Schumacher,
{\it Harmonic maps of the moduli space of compact Riemann surfaces},
Math. Ann., {\bf 275}: 455-466 (1986).

\bibitem{bib14}
D. Mumford,
{\it A remark on Mahler's compactness theorem},
Proc. Amer. Math. Soc., {\bf 28}: 289-294 (1971).

\bibitem{bib15}
S.-T. Yau,
{\it Nonlinear analysis in geometry},
L'Enseig. Math., {\bf 33}: 109-158 (1987).

\bibitem{bib16}
S.-T. Yau,
{\it A general Schwarz lemma for K\"{a}hler manifolds},
Amer. J. Math., {\bf 100}(1): 197-203 (1978).

\bibitem{bib17}
S. Y. Cheng and S.-T. Yau,
{\it On the existence of a complete Kahler metric on noncompact complex manifolds and the regularity of Feffermans equation},
Comm. Pure Appl. Math., {\bf 33}(4): 507-544 (1980).

\bibitem{bib18}
N. Mok and S.-T. Yau,
{\it Completeness of the K\"{a}hler-Einstein metric on bounded domains and the characterization of domains of holomorphy by curvature conditions},
The Mathematical Heritage of Henri Poincar\'{e}, Proc. of Symp. in Pure Math., Amer. Math. Soc., 1983, pp. 41-59.

\bibitem{bib19}
L. Bers and L. Ehrenpreis,
{\it Holomorphic Convexity of Teichm\"{u}ller Spaces},
Bull. Amer. Math. Soc., {\bf 70}: 761-764 (1964).

\bibitem{bib20}
L. Bers,
{\it Spaces of Riemann Surfaces as Bounded Domains},
Bull. Amer. Math. Soc., {\bf 66}: 98-103 (1960).

\bibitem{bib21}
L. Bers,
{\it Correction to "Spaces of Riemann Surfaces as Bounded Domains"},
Bull. Amer. Math. Soc., {\bf 67}: 465-466 (1961).

\bibitem{bib22}
L. V. Ahlfors,
{\it Lectures on Quasiconformal Mappings},
Van Nostrand-Reinhold, Princeton, New Jersey, 1966.

\bibitem{bib23}
O. Lehto and K. I. Virtanen,
{\it Quasiconformal Mappings},
Springer-Verlag, Berlin and New York, 1965.

\bibitem{bib24}
L. V. Ahlfors and L. Bers,
{\it Riemann's Mapping Theorem for Variable Metrics},
Ann. Math., {\bf 72}: 385-404 (1960).

\bibitem{bib25}
F. P. Gardiner,
{\it Teichm\"{u}ller Theory and Quadratic Differentials},
John Wiley \& Sons, 1987.

\bibitem{bib26}
L. Keen,
{\it Collars on Riemann Surfaces},
Discontinuous Groups and Riemann Surfaces (Proc. Conf. Univ. Maryland, College Park, Maryland, 1973), Ann. of Math. Studies No.79, Princeton Univ. Press, Princeton, New Jersey, 1974, pp. 263-268. 

\bibitem{bib27}
H. L. Royden,
{\it Automorphisms and Isometries of Teichm\"{u}ller Space},
Ann. Math. Stud., {\bf 66}: 369-384 (1971).

\bibitem{bib28}
S. Kobayashi,
{\it Hyperbolic Complex Spaces},
Grundlehren der Mathematischen Wissenschaften Volume 318, Springer-Verlag, Berlin, 1998.

\bibitem{bib29}
S. A. Wolpert,
{\it Chern forms and the Riemann tensor for the moduli space of curves},
Invent. Math., {\bf 85}(1): 119-145 (1986).

\bibitem{bib30}
G. Schumacher,
{\it The curvature of the Petersson-Weil metric on the moduli space of K\"{a}hler-Einstein manifolds},
Complex Analysis and Geometry, Univ Ser. Math., Plenum, New York, 1993, pp. 339-354.

\bibitem{bib31}
Y. T. Siu,
{\it Curvature of the Weil-Petersson metric in the moduli space of compact K\"{a}hler-Einstein manifolds of negative first Chern class},
Contributions to Several Complex Variables, Aspects Math., E9, Vieweg, Braunschweig, 1986, pp. 261-298.

\bibitem{bib32}
Y. Imayoshi and M. Taniguchi,
{\it An Introduction to Teichm\"{u}ller Spaces},
Springer-Verlag, Tokyo, 1992.

\bibitem{bib33}
P. Deligne and D. Mumford,
{\it The irreducibility of the space of curves of given genus},
Inst. Hautes \'{E}tudes Sci. Publ. Math., {\bf 36}: 75-109, 1969.

\end{thebibliography}

